Retrieval-Guided Reinforcement Learning for Boolean Circuit Minimization

Logic synthesis, a pivotal stage in chip design, entails optimizing chip specifications encoded in hardware description languages like Verilog into highly efficient implementations using Boolean logic gates. The process involves a sequential application of logic minimization heuristics (``synthesis recipe"), with their arrangement significantly impacting crucial metrics such as area and delay. Addressing the challenge posed by the broad spectrum of design complexities - from variations of past designs (e.g., adders and multipliers) to entirely novel configurations (e.g., innovative processor instructions) - requires a nuanced `synthesis recipe` guided by human expertise and intuition. This study conducts a thorough examination of learning and search techniques for logic synthesis, unearthing a surprising revelation: pre-trained agents, when confronted with entirely novel designs, may veer off course, detrimentally affecting the search trajectory. We present ABC-RL, a meticulously tuned $\alpha$ parameter that adeptly adjusts recommendations from pre-trained agents during the search process. Computed based on similarity scores through nearest neighbor retrieval from the training dataset, ABC-RL yields superior synthesis recipes tailored for a wide array of hardware designs. Our findings showcase substantial enhancements in the Quality-of-result (QoR) of synthesized circuits, boasting improvements of up to 24.8% compared to state-of-the-art techniques. Furthermore, ABC-RL achieves an impressive up to 9x reduction in runtime (iso-QoR) when compared to current state-of-the-art methodologies.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/rebuttal_tab1.tex <==
\newpage

\begin{wrapfigure}[16]{r}{0.5\textwidth}
\centering
\setlength\tabcolsep{3.5pt}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lrrrrrr}
\toprule
\multirow{3}{*}{Designs}& \multicolumn{5}{c}{ADP reduction (in \%)} & \multirow{3}{*}{\begin{tabular}{@{}c@{}}Iso-\\ADP\\Speed-\\Up\end{tabular}} \\
\cmidrule(lr){2-6}
& \multirow{2}{*}{\begin{tabular}{@{}c@{}}Online-\\RL\\\cite{mlcad_abc}\end{tabular}}& \multirow{2}{*}{\begin{tabular}{@{}c@{}}SA+\\Pred.\\\cite{bullseye}\end{tabular}} & \multirow{2}{*}{\begin{tabular}{@{}c@{}}MCTS\\\cite{neto2022flowtune}\end{tabular}} &
\multicolumn{2}{c}{\solution{}} & \\
\cmidrule(lr){5-6}
& & & & $\alpha=1$ & +OOD & \\
\midrule
arbiter & \textbf{0.03} & \textbf{0.03} & \textbf{0.03} & \textbf{0.03} &  \textbf{0.03}(\cmark) & 2.4x\\
cavlc & 16.28 & \textbf{16.75} & 15.85 & 13.89 & 15.85(\xmark) & 1.0x\\
ctrl & 22.97 & 25.85 & 27.58 & \textbf{30.85} & \textbf{30.85}(\cmark) & 2.6x \\
i2c & 14.91 & 13.10 & 13.45 & \textbf{15.65} & \textbf{15.65}(\cmark) & 3.0x \\
int2float & 7.41 & 7.52 & \textbf{8.10} & 7.52 & \textbf{8.10}(\xmark) & 1.0x \\
mem\_ctrl & 22.54 & 21.45 & 21.55 & \textbf{23.67} & \textbf{23.67}(\cmark) & 2.1x\\
priority & 74.62 & 77.10 & \textbf{77.53} & 75.10 & \textbf{77.53}(\xmark)& 1.0x\\
router & 10.71 & 27.53 & 21.63 & \textbf{25.68}  & 21.63(\xmark) & 1.0x \\
voter & 8.26 & 26.45 & \textbf{27.10} & 26.05 & \textbf{27.10}(\xmark) & 1.0x \\
\midrule
Geomean & 8.29 & 10.47 & 10.38 & 10.69 & \textbf{10.80} & 1.5x \\
Win ratio & 0/9 & 2/9 & 4/9 & 5/9 & 7/9 & 4/9\\
\bottomrule
\end{tabular}
}
    \captionof{table}{Area-delay reduction compared to \texttt{resyn2} on EPFL random-control benchmarks. \cmark denotes \solution{} deploy agent guided search whereas {\xmark} denotes standard MCTS}
\label{tab:rebuttal1}
\end{wrapfigure}

==> tables/table_ablation.tex <==

\begin{wrapfigure}[9]{r}{0.5\textwidth}
\centering
\setlength\tabcolsep{3.5pt}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lrrrrrr}
\toprule
\multirow{2}{*}{ Settings } & \multicolumn{2}{c}{MCNC} & \multicolumn{2}{c}{EPFL arith} & \multicolumn{2}{c}{EPFL random} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
& G.M. & W.R. & G.M & W.R. & G.M. & W.R. \\
\midrule
$\alpha=1$ & 18.84 & 8/12 & 21.46 & 8/9 & 10.78 & 5/9 \\
$T=0$ & 19.76 & 10/12 & 22.07 & 9/9 & 10.80 & 7/9 \\
$T=0.06$ & 20.41 & 11/12 & 21.63 & 8/9 & 11.32 & 7/9 \\
\bottomrule
\end{tabular}
}
\captionof{table}{Varying agent's recommendation during search}%\cmark denotes \solution{} used RL agent during search whereas {\xmark} denotes standard MCTS}
\label{tab:ablation}
\end{wrapfigure}

==> tables/table_combinedAgent.tex <==
% \begin{table}[!tbh]
% \centering
% \setlength\tabcolsep{2.9pt}
% \caption{Area-delay improvement}
% \label{tab:qorOfAgents}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|rrrrrrrrrrrr|rrrr|rrrr}
% \toprule
% \multirow{3}{*}{Methods}& \multicolumn{20}{c}{ADP improvement (in \%)} \\
% \cmidrule(lr){2-21}
% &  \multicolumn{12}{c|}{MCNC} & \multicolumn{4}{c|}{EPFL arith} & \multicolumn{4}{c}{EPFL random} \\
% \cmidrule(lr){2-13}\cmidrule(lr){14-17}\cmidrule(lr){18-21}
% & alu4 & apex1 & apex2 & apex4 & i9 & m4 & prom1 & b9 & c880 & c7552 & pair & max1024 & bar & div & square & sqrt & cavlc & mem\_ctrl & router & voter \\ 
% \midrule
% \specialcell{\cite{mlcad_abc}} & 20.61 & 6.58 & 8.12 & 13.53 & 39.38 & 20.95 & 4.97 & 17.92 & 16.23 & 20.21 & 4.73 & 11.39 & 36.89 & 34.83 & 10.44 & 24.10 & 16.28 & 22.54 & 10.71 & 8.26\\
% \specialcell{\cite{bullseye}} & 17.58 & 17.01 & 15.58 & 13.01 & 46.45 & 18.16 & 8.53 & 23.65 & \bbt{19.95} & 17.62 & 10.02 & 20.27 & 36.89 & 25.16 & 8.20 & 21.10 & 16.75 & 21.45 & 25.68 & 26.15\\
% \specialcell{\cite{neto2022flowtune}} & 17.05 & 15.95 & 13.06 & 13.01 & 46.89 & 14.98 & 6.50 & 23.21 & 17.74 & \bbt{20.45} & 13.10 & 19.65 & 25.37 & 45.94 & 10.71 & 18.69 & 15.85 & 21.55 & 21.63 & \bbt{27.10}\\
% \midrule
% \solution{} & 19.95 & \rbt{19.59} & {16.80} & \rbt{14.95} & {46.89} & \bbt{19.10} & \rbt{12.10} & \rbt{24.30} & \bbt{21.25} & \rbt{21.12} & \bbt{13.55} & \bbt{21.58} & {36.89} & \rbt{56.15} & \rbt{14.00} & \rbt{23.75} & \rbt{19.75} & \rbt{30.20} & \rbt{38.85} & \rbt{30.04} 
% \\
% \solution{} solo & \bbt{20.84} & \bbt{19.23} & \bbt{17.48} & \rbt{14.95} & \bbt{52.45} & 18.10 & 10.89 & 24.10 & \rbt{24.70} & \rbt{21.12} & \rbt{16.75} & \rbt{21.95} & 36.89 & \bbt{55.89} & \bbt{12.05} & \rbt{25.14} & \bbt{17.77} & 22.75 & 26.55 & \bbt{27.10} \\
% \midrule
% \solution{} w/o $\alpha$ tune & 16.97 & \rbt{19.59} & 16.90 & 12.45 & 46.85 & 13.87 & 10.12 & 24.10 & 17.10 & 16.75 & 8.10 & 19.45 & 36.89 & \bbt{55.89} & 10.25 & 22.65 & 15.75 & \bbt{24.10} & \rbt{38.85} & 26.85  \\
% \solution{} solo w/o $\alpha$ tune & \rbt{21.95} & 17.54 & \rbt{17.51} & \bbt{13.95} & \rbt{53.97} & \rbt{20.05} & 11.12 & 24.10 & 12.78 & \bbt{20.45} & 12.65 & 18.32 & 36.89 & 55.64 & 9.75 & \bbt{24.84} & 13.89 & 23.67 & 25.68 & 26.05 \\
% \solution{} w/o BERT & 17.01 & 16.50 & 14.87 & 13.10 & 44.58 & 16.85 & 10.01 & 23.45 & 16.28 & 18.77 & 10.55 & 18.95 & 36.89 & 51.66 & 9.85 & 20.03 & 15.50 & 22.96 & 27.95 & 26.85 \\
% \bottomrule
% \end{tabular}
% }
% \end{table}









% \begin{table}[!tbh]
% \centering
% \caption{Area-delay reduction on EPFL arithmetic benchmarks. \cmark denotes \solution{} used RL agent during search whereas {\xmark} denotes Flowtune (Blind MCTS search). $K$ denotes number of iterations post which winner thread is picked}
% \label{tab:qorEPFLarith}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lrrrccccrrrr}
% \toprule
% \multirow{2}{*}{Benchmarks}& \multicolumn{3}{c}{ADP reduction(\%)} & \multicolumn{4}{c}{Pre-trained agent used?} & \multicolumn{4}{c}{ADP reduction(\%)} \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-8} \cmidrule(lr){9-12}
% &  MCTS & \specialcell{MCTS\\$+$RL} & Bulls-eye & \specialcell{Zero\\(cosine)} & \specialcell{Low\\(k=20)} & \specialcell{Mid\\(k=40)} & \specialcell{High\\(k=60)} & \specialcell{Zero\\(cosine)} & \specialcell{Low\\(k=20)} & \specialcell{Mid\\(k=40)} & \specialcell{High\\(k=60)} \\
% \midrule
% adder & \textbf{18.63} & \textbf{18.63} & \textbf{18.63} & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{18.63} & \textbf{18.63} & \textbf{18.63} & \textbf{18.63}\\
% bar & 25.37 & \textbf{36.89} & \textbf{36.89} & {\cmark} & {\xmark} & {\cmark} & {\cmark} & \textbf{36.89} & 25.37 & \textbf{36.89} & \textbf{36.89} \\
% div & 45.94 & \textbf{55.64} & 25.16  & {\cmark} & {\xmark} & {\xmark} & {\cmark} & \textbf{55.64} & 45.94 & 45.94 & \textbf{55.64} \\
% log2 & 9.09 & \textbf{11.51} & 9.58 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{11.51} & \textbf{11.51} & \textbf{11.51} & \textbf{11.51}\\
% max & 37.5 & \textbf{46.86} & 29.87 & {\cmark} & {\cmark} & {\xmark} & {\cmark} & \textbf{46.86} & \textbf{46.86} & 37.5 & \textbf{46.86}\\
% multiplier & 9.9 & \textbf{12.68} & 9.75 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{12.68} & \textbf{12.68} & \textbf{12.68} & \textbf{12.68} \\
% sin & 14.50 & \textbf{15.96} & 14.30 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{15.96} & \textbf{15.96} & \textbf{15.96} & \textbf{15.96} \\
% square & \textbf{12.28} & 9.75 & 8.20 & {\xmark} & {\cmark} & {\cmark} & {\xmark} & \textbf{12.28} & 9.75 & 9.75 & \textbf{12.28} \\
% sqrt & 18.69 & \textbf{24.24} & 21.10 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{24.24} & \textbf{24.24} & \textbf{24.24} & \textbf{24.24}  \\
% \midrule
% Geomean & 18.42 & 21.51 & 17.01 & & & & & \textbf{\rt{22.07}} & 20.20 & \textbf{\bt{20.54}} & \textbf{\rt{22.07}} \\
% Win ratio & 2/9 & 8/9 & 2/9 & &  &  &  & 9/9 & 6/9 & 6/9 & 9/9\\
% \bottomrule
% \end{tabular}
% }

% \end{table}





==> tables/table_epfl_arith.tex <==
% \begin{table}[!tbh]
% \centering
% \caption{Area-delay improvement on EPFL arithmetic benchmarks. \gt{\cmark} denotes \solution{} wins with MCTS+RL agent wheras \ot{\cmark} denotes winning by MCTS search only. K=20(Low), 40(Mid) and 60(High) efforts post which winner is picked}
% \label{tab:qorOfAgents}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lrrrrrrrrr}
% \toprule
% \multirow{2}{*}{Benchmarks}& \multicolumn{5}{c}{ADP improvement (in \%)} & \multicolumn{4}{c}{\solution{} as winner} \\
% \cmidrule(lr){2-6}\cmidrule(lr){7-10}
% & Flowtune & Zero & Low & Mid & High & Zero & Low & Mid & High \\
% \midrule
% adder & 18.63 & 18.63 & 18.63 & 18.63 & 18.63 & \gt{\cmark} & \gt{\cmark} & \gt{\cmark} & \gt{\cmark} \\
% bar & 25.37 & 36.89 & 25.37 & 36.89 & 36.89 & \gt{\cmark} & \rt{\xmark} & \gt{\cmark} & \gt{\cmark} \\
% div & 45.94 & 45.94 & 45.94 & 55.64 & 55.64 & \gt{\cmark} & \rt{\xmark} & \gt{\cmark} & \gt{\cmark} \\
% log2 & 9.09 & 11.51 & 11.51 & 11.51 & 11.51 & \gt{\cmark} & \gt{\cmark} & \gt{\cmark} & \gt{\cmark} \\
% max & 37.5 & 37.5 & 41.86 & 37.5 & 41.86 & \gt{\cmark} & \gt{\cmark} & \rt{\xmark} & \gt{\cmark} \\
% multiplier & 9.9 & 12.68 & 12.68 & 9.9 & 12.68 & \gt{\cmark} & \gt{\cmark} & \rt{\xmark} & \gt{\cmark} \\
% sin & 14.5 & 15.96 & 15.96 & 15.96 & 15.96 & \gt{\cmark} & \gt{\cmark} & \gt{\cmark} & \gt{\cmark} \\
% square & 12.28 & 12.28 & 8.25 & 8.25 & 12.28 & \ot{\cmark} & \rt{\xmark} & \rt{\xmark} & \ot{\cmark} \\
% sqrt & 18.69 & 24.24 & 24.24 & 24.24 & 24.24 & \gt{\cmark} & \gt{\cmark} & \gt{\cmark} & \gt{\cmark} \\
% \bottomrule
% \end{tabular}
% }

% \end{table}

% \begin{table}[!tbh]
% \centering
% \caption{Area-delay reduction on EPFL arithmetic benchmarks. \cmark denotes \solution{} used RL agent during search whereas {\xmark} denotes Flowtune (Blind MCTS search). $K$ denotes number of iterations post which winner thread is picked}
% \label{tab:qorEPFLarith}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lrrrccccrrrr}
% \toprule
% \multirow{2}{*}{Benchmarks}& \multicolumn{3}{c}{ADP reduction(\%)} & \multicolumn{4}{c}{Pre-trained agent used?} & \multicolumn{4}{c}{ADP reduction(\%)} \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-8} \cmidrule(lr){9-12}
% &  MCTS & \specialcell{MCTS\\$+$RL} & Bulls-eye & \specialcell{Zero\\(cosine)} & \specialcell{Low\\(k=20)} & \specialcell{Mid\\(k=40)} & \specialcell{High\\(k=60)} & \specialcell{Zero\\(cosine)} & \specialcell{Low\\(k=20)} & \specialcell{Mid\\(k=40)} & \specialcell{High\\(k=60)} \\
% \midrule
% adder & \textbf{18.63} & \textbf{18.63} & \textbf{18.63} & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{18.63} & \textbf{18.63} & \textbf{18.63} & \textbf{18.63}\\
% bar & 25.37 & \textbf{36.89} & \textbf{36.89} & {\cmark} & {\xmark} & {\cmark} & {\cmark} & \textbf{36.89} & 25.37 & \textbf{36.89} & \textbf{36.89} \\
% div & 45.94 & \textbf{55.64} & 25.16  & {\cmark} & {\xmark} & {\xmark} & {\cmark} & \textbf{55.64} & 45.94 & 45.94 & \textbf{55.64} \\
% log2 & 9.09 & \textbf{11.51} & 9.58 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{11.51} & \textbf{11.51} & \textbf{11.51} & \textbf{11.51}\\
% max & 37.5 & \textbf{46.86} & 29.87 & {\cmark} & {\cmark} & {\xmark} & {\cmark} & \textbf{46.86} & \textbf{46.86} & 37.5 & \textbf{46.86}\\
% multiplier & 9.9 & \textbf{12.68} & 9.75 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{12.68} & \textbf{12.68} & \textbf{12.68} & \textbf{12.68} \\
% sin & 14.50 & \textbf{15.96} & 14.30 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{15.96} & \textbf{15.96} & \textbf{15.96} & \textbf{15.96} \\
% square & \textbf{12.28} & 9.75 & 8.20 & {\xmark} & {\cmark} & {\cmark} & {\xmark} & \textbf{12.28} & 9.75 & 9.75 & \textbf{12.28} \\
% sqrt & 18.69 & \textbf{24.24} & 21.10 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{24.24} & \textbf{24.24} & \textbf{24.24} & \textbf{24.24}  \\
% \midrule
% Geomean & 18.42 & 21.51 & 17.01 & & & & & \textbf{\rt{22.07}} & 20.20 & \textbf{\bt{20.54}} & \textbf{\rt{22.07}} \\
% Win ratio & 2/9 & 8/9 & 2/9 & &  &  &  & 9/9 & 6/9 & 6/9 & 9/9\\
% \bottomrule
% \end{tabular}
% }

% \end{table}


% \begin{table}[!tbh]
% \centering
% \caption{Area-delay reduction on EPFL arithmetic benchmarks. \cmark denotes \solution{} used RL agent during search whereas {\xmark} denotes Flowtune (Blind MCTS search). $K$ denotes number of iterations post which winner thread is picked}
% \label{tab:qorEPFLarith}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lrrrccccrrrr}
% \toprule
% \multirow{2}{*}{Benchmarks}& \multicolumn{3}{c}{ADP reduction(\%)} & \multicolumn{4}{c}{Pre-trained agent used?} & \multicolumn{4}{c}{ADP reduction(\%)} \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-8} \cmidrule(lr){9-12}
% &  MCTS & \specialcell{MCTS\\$+$RL} & Bulls-eye & \specialcell{Zero\\(cosine)} & \specialcell{Low\\(k=20)} & \specialcell{Mid\\(k=40)} & \specialcell{High\\(k=60)} & \specialcell{Zero\\(cosine)} & \specialcell{Low\\(k=20)} & \specialcell{Mid\\(k=40)} & \specialcell{High\\(k=60)} \\
% \midrule
% adder & \textbf{18.63} & \textbf{18.63} & \textbf{18.63} & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{18.63} & \textbf{18.63} & \textbf{18.63} & \textbf{18.63}\\
% bar & 25.37 & \textbf{36.89} & \textbf{36.89} & {\cmark} & {\xmark} & {\cmark} & {\cmark} & \textbf{36.89} & 25.37 & \textbf{36.89} & \textbf{36.89} \\
% div & 45.94 & \textbf{55.64} & 25.16  & {\cmark} & {\xmark} & {\xmark} & {\cmark} & \textbf{55.64} & 45.94 & 45.94 & \textbf{55.64} \\
% log2 & 9.09 & \textbf{11.51} & 9.58 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{11.51} & \textbf{11.51} & \textbf{11.51} & \textbf{11.51}\\
% max & 37.5 & \textbf{46.86} & 29.87 & {\cmark} & {\cmark} & {\xmark} & {\cmark} & \textbf{46.86} & \textbf{46.86} & 37.5 & \textbf{46.86}\\
% multiplier & 9.9 & \textbf{12.68} & 9.75 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{12.68} & \textbf{12.68} & \textbf{12.68} & \textbf{12.68} \\
% sin & 14.50 & \textbf{15.96} & 14.30 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{15.96} & \textbf{15.96} & \textbf{15.96} & \textbf{15.96} \\
% square & \textbf{12.28} & 9.75 & 8.20 & {\xmark} & {\cmark} & {\cmark} & {\xmark} & \textbf{12.28} & 9.75 & 9.75 & \textbf{12.28} \\
% sqrt & 18.69 & \textbf{24.24} & 21.10 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{24.24} & \textbf{24.24} & \textbf{24.24} & \textbf{24.24}  \\
% \midrule
% Geomean & 18.42 & 21.51 & 17.01 & & & & & \textbf{\rt{22.07}} & 20.20 & \textbf{\bt{20.54}} & \textbf{\rt{22.07}} \\
% Win ratio & 2/9 & 8/9 & 2/9 & &  &  &  & 9/9 & 6/9 & 6/9 & 9/9\\
% \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{wrapfigure}{r}{0.5\textwidth}
\centering
\setlength\tabcolsep{3.5pt}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lrrrrrr}
\toprule
\multirow{3}{*}{Designs}& \multicolumn{5}{c}{ADP reduction (in \%)} & \multirow{3}{*}{\begin{tabular}{@{}c@{}}Iso-\\ADP\\Speed-\\Up\end{tabular}} \\
\cmidrule(lr){2-6}
& \multirow{2}{*}{\begin{tabular}{@{}c@{}}Online-\\RL\\\cite{mlcad_abc}\end{tabular}}& \multirow{2}{*}{\begin{tabular}{@{}c@{}}SA+\\Pred.\\\cite{bullseye}\end{tabular}} & \multirow{2}{*}{\begin{tabular}{@{}c@{}}MCTS\\\cite{neto2022flowtune}\end{tabular}} &
\multicolumn{2}{c}{\solution{}} & \\
\cmidrule(lr){5-6}
& & & & $\alpha=1$ & +OOD & \\
\midrule
adder & \textbf{18.63} & \textbf{18.63} & \textbf{18.63} & \textbf{18.63} &  \textbf{18.63}(\cmark) & 2.2x\\
bar & \textbf{36.89} & \textbf{36.89} & 25.37 & \textbf{36.89} & \textbf{36.89}(\cmark) & 0.6x\\
div & 34.83 & 25.16 & 45.94 & \textbf{55.64} & \textbf{55.64}(\cmark) & 1.4x\\
log2 & 4.73 & 9.58 & 9.09 & \textbf{11.51} & \textbf{11.51}(\cmark) & 1.9x \\
max & 25.09 & 29.87 & 37.50 & \textbf{46.86} & \textbf{46.86}(\cmark) & 1.2x \\
multiplier & 12.41 & 9.75 & 9.90 & \textbf{12.68} & \textbf{12.68}(\cmark) & 1.4x \\
sin & 5.57 & 14.30 & 14.50 & \textbf{15.96} & \textbf{15.96}(\cmark) & 2.4x \\
square & 10.44 & 8.20 & \textbf{12.28} & 9.75  &\textbf{12.28}(\xmark) & 1.0x\\
sqrt & 24.10 & 21.10 & 18.69 & \textbf{24.24} & \textbf{24.24}(\cmark) & 6.3x\\
\midrule
Geomean& 15.41 & 17.01 & 18.42 & 21.51 & \textbf{22.07} & 1.6x\\
Win ratio & 2/9 & 2/9 & 2/9 & 8/9 & 9/9 & 7/9 \\
\bottomrule
\end{tabular}
}
    \captionof{table}{Area-delay reduction over \texttt{resyn2} on EPFL arithmetic benchmarks. \cmark denotes \solution{} perform agent guided search whereas {\xmark} denotes standard MCTS}
\label{tab:qorEPFLarith}
\end{wrapfigure}


% \begin{wrapfigure}{r}{0.5\textwidth}
% \centering
% \setlength\tabcolsep{3.5pt}
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{lrrrrr}
% \toprule
% \multirow{3}{*}{Designs}& \multicolumn{4}{c}{ADP reduction (in \%)} \\
% \cmidrule(lr){2-6}
% & \multirow{2}{*}{\begin{tabular}{@{}c@{}}on-\\policy\\\cite{mlcad_abc}\end{tabular}}& \multirow{2}{*}{\begin{tabular}{@{}c@{}}SA+\\Pred.\\\cite{bullseye}\end{tabular}} &
% \multicolumn{3}{c}{MCTS}\\
% \cmidrule(lr){4-6}
% & & & \specialcell{$\alpha=0$\\\cite{neto2022flowtune}} & $\alpha=1$ & \specialcell{OOD\\(\solution{})}\\
% \midrule
% adder & \textbf{18.63} & \textbf{18.63} & \textbf{18.63} & \textbf{18.63} &  \textbf{18.63}(\cmark) \\
% bar & \textbf{36.89} & \textbf{36.89} & 25.37 & \textbf{36.89} & \textbf{36.89}(\cmark)\\
% div & 34.83 & 25.16 & 45.94 & \textbf{55.64} & \textbf{55.64}(\cmark) \\
% log2 & 4.73 & 9.58 & 9.09 & \textbf{11.51} & \textbf{11.51}(\cmark) \\
% max & 25.09 & 29.87 & 37.50 & \textbf{46.86} & \textbf{46.86}(\cmark)\\
% multiplier & 12.41 & 9.75 & 9.90 & \textbf{12.68} & \textbf{12.68}(\cmark)\\
% sin & 5.57 & 14.30 & 14.50 & \textbf{15.96} & \textbf{15.96}(\cmark)\\
% square & 10.44 & 8.20 & \textbf{12.28} & 9.75  &\textbf{12.28}(\xmark)\\
% sqrt & 24.10 & 21.10 & 18.69 & \textbf{24.24} & \textbf{24.24}(\cmark) \\
% \midrule
% Geomean & 15.41 & 17.01 & 18.42 & 21.51 & \textbf{22.07} \\
% Win ratio & 2/9 & 2/9 & 2/9 & 8/9 & 9/9 \\
% \bottomrule
% \end{tabular}
% }
%     \captionof{table}{Area-delay reduction over \texttt{resyn2} on EPFL arithmetic benchmarks. \cmark denotes \solution{} perform agent guided search whereas {\xmark} denotes standard MCTS}
% \label{tab:qorEPFLarith}
% \end{wrapfigure}


% \begin{wrapfigure}{r}{0.4\textwidth}
% \centering
% \setlength\tabcolsep{3.5pt}
% \resizebox{0.4\textwidth}{!}{%
% \begin{tabular}{lrrrr}
% \toprule
% \multirow{2}{*}{Designs}& \multicolumn{3}{c}{ADP reduction (in \%)} \\
% \cmidrule(lr){2-5}
% & \specialcell{on-\\policy\\\cite{mlcad_abc}} & \specialcell{SA+\\Pred.\\\cite{bullseye}} & \specialcell{MCTS\\\cite{neto2022flowtune}} & \specialcell{\textbf{Ours}} \\
% \midrule
% adder & \textbf{18.63} & \textbf{18.63} & \textbf{18.63}  &  \textbf{18.63} \\
% bar & \textbf{36.89} & \textbf{36.89} & 25.37 & \textbf{36.89}\\
% div & 34.83 & 25.16 & 45.94 & \textbf{55.89}\\
% log2 & 4.73 & 9.58 & 9.09 & \textbf{11.38} \\
% max & 25.09 & 29.87 & 37.50 & \textbf{43.05}\\
% multiplier & 12.41 & 9.75 & 9.90 & \textbf{13.05}\\
% sin & 5.57 & 14.30 & 14.50 & \textbf{15.75}\\
% square & 10.44 & 8.20 & 10.71 & \textbf{10.73}\\
% sqrt & 24.10 & 21.10 & 18.69 & \textbf{25.04} \\
% \midrule
% Geomean & 15.41 & 17.01 & 18.13 & \textbf{21.63} \\
% Win ratio & 2/9 & 2/9 & 2/9 & 9/9 \\
% \bottomrule
% \end{tabular}
% }
%     \captionof{table}{Area-delay reduction over \texttt{resyn2} on EPFL arithmetic benchmarks.}%\cmark denotes \solution{} used RL agent during search whereas {\xmark} denotes standard MCTS}
% \label{tab:qorEPFLarith}
% \end{wrapfigure}



==> tables/table_epfl_rc.tex <==
% \begin{table}[!tbh]
% \centering
% \caption{Area-delay reduction on EPFL random control benchmarks. \cmark denotes \solution{} used RL agent during search whereas {\xmark} denotes Flowtune (Blind MCTS search). $K$ denotes number of iterations post which winner thread is picked}
% \label{tab:qorEPFLrc}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lrrrccccrrrr}
% \toprule
% \multirow{2}{*}{Benchmarks}& \multicolumn{3}{c}{ADP reduction(\%)} & \multicolumn{4}{c}{Pre-trained agent used?} & \multicolumn{4}{c}{ADP reduction(\%)} \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-8} \cmidrule(lr){9-12}
% &  MCTS & \specialcell{MCTS\\$+$RL} & Bulls-eye  & \specialcell{Zero\\(cosine)} & \specialcell{Low\\(k=20)} & \specialcell{Mid\\(k=40)} & \specialcell{High\\(k=60)} & \specialcell{Zero\\(cosine)} & \specialcell{Low\\(k=20)} & \specialcell{Mid\\(k=40)} & \specialcell{High\\(k=60)} \\
% \midrule
% arbiter & \textbf{0.03} & \textbf{0.03} & \textbf{0.03} & {\cmark} & {\xmark} & {\cmark} & {\cmark} & \textbf{0.03} & \textbf{0.03} & \textbf{0.03} & \textbf{0.03}\\
% cavlc & 15.85 & 13.89 & \textbf{16.75} & {\xmark} & {\cmark} & {\xmark} & {\xmark} & 15.85 & 13.89 & 15.85 & 15.85 \\
% ctrl & 27.58 & \textbf{30.85} & 25.85 & {\cmark} & {\xmark} & {\cmark} & {\cmark} & \textbf{30.85} & 27.58 & \textbf{30.85} & \textbf{30.85} \\
% i2c & 13.45 & \textbf{15.65} & 13.10 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{15.65} & \textbf{15.65} & \textbf{15.65} & \textbf{15.65}\\
% int2float & \textbf{8.10} & 7.65 & 7.52 & {\xmark} & {\cmark} & {\xmark} & {\xmark} & \textbf{8.10} & 7.65 & \textbf{8.10} & \textbf{8.10}\\
% mem\_ctrl & 21.55 & \textbf{23.67} & 21.45 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{23.67} & \textbf{23.67} & \textbf{23.67} & \textbf{23.67} \\
% priority & \textbf{77.53} & 75.10 & 77.10 & {\xmark} & {\xmark} & {\cmark} & {\xmark} & \textbf{77.53} & \textbf{77.53} & 75.10 & \textbf{77.53} \\
% router & 21.63 & \textbf{27.68} & 27.53 & {\xmark} & {\cmark} & {\cmark} & {\cmark} & 21.63 & \textbf{27.68} & \textbf{27.68} & \textbf{27.68} \\
% voter & \textbf{27.10} & 26.05 & 26.45 &{\xmark} & {\xmark} & {\xmark} & {\xmark} & \textbf{27.10} & \textbf{27.10} & \textbf{27.10} & \textbf{27.10}  \\
% \midrule
% Geomean & 10.38 & 10.78 & 10.47 & & & & & 10.80 & 10.74 & \textbf{\bt{11.06}} & \textbf{\rt{11.10}} \\
% Win ratio & 4/9 & 5/9 & 2/9 & &  &  &  & 7/9 & 6/9 & 7/9 & 8/9\\
% \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{wrapfigure}[16]{r}{0.5\textwidth}
\centering
\setlength\tabcolsep{3.5pt}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lrrrrrr}
\toprule
\multirow{3}{*}{Designs}& \multicolumn{5}{c}{ADP reduction (in \%)} & \multirow{3}{*}{\begin{tabular}{@{}c@{}}Iso-\\ADP\\Speed-\\Up\end{tabular}} \\
\cmidrule(lr){2-6}
& \multirow{2}{*}{\begin{tabular}{@{}c@{}}Online-\\RL\\\cite{mlcad_abc}\end{tabular}}& \multirow{2}{*}{\begin{tabular}{@{}c@{}}SA+\\Pred.\\\cite{bullseye}\end{tabular}} & \multirow{2}{*}{\begin{tabular}{@{}c@{}}MCTS\\\cite{neto2022flowtune}\end{tabular}} &
\multicolumn{2}{c}{\solution{}} & \\
\cmidrule(lr){5-6}
& & & & $\alpha=1$ & +OOD & \\
\midrule
arbiter & \textbf{0.03} & \textbf{0.03} & \textbf{0.03} & \textbf{0.03} &  \textbf{0.03}(\cmark) & 2.4x\\
cavlc & 16.28 & \textbf{16.75} & 15.85 & 13.89 & 15.85(\xmark) & 1.0x\\
ctrl & 22.97 & 25.85 & 27.58 & \textbf{30.85} & \textbf{30.85}(\cmark) & 2.6x \\
i2c & 14.91 & 13.10 & 13.45 & \textbf{15.65} & \textbf{15.65}(\cmark) & 3.0x \\
int2float & 7.41 & 7.52 & \textbf{8.10} & 7.52 & \textbf{8.10}(\xmark) & 1.0x \\
mem\_ctrl & 22.54 & 21.45 & 21.55 & \textbf{23.67} & \textbf{23.67}(\cmark) & 2.1x\\
priority & 74.62 & 77.10 & \textbf{77.53} & 75.10 & \textbf{77.53}(\xmark)& 1.0x\\
router & 10.71 & 27.53 & 21.63 & \textbf{25.68}  & 21.63(\xmark) & 1.0x \\
voter & 8.26 & 26.45 & \textbf{27.10} & 26.05 & \textbf{27.10}(\xmark) & 1.0x \\
\midrule
Geomean & 8.29 & 10.47 & 10.38 & 10.69 & \textbf{10.80} & 1.5x \\
Win ratio & 0/9 & 2/9 & 4/9 & 5/9 & 7/9 & 4/9\\
\bottomrule
\end{tabular}
}
    \captionof{table}{Area-delay reduction compared to \texttt{resyn2} on EPFL random-control benchmarks. \cmark denotes \solution{} deploy agent guided search whereas {\xmark} denotes standard MCTS}
\label{tab:qorEPFLrc}
\end{wrapfigure}

% \begin{wrapfigure}{r}{0.4\textwidth}
% \centering
% \setlength\tabcolsep{3.5pt}
% \resizebox{0.4\textwidth}{!}{%
% \begin{tabular}{lrrrr}
% \toprule
% \multirow{2}{*}{Designs}& \multicolumn{4}{c}{ADP reduction (in \%)} \\
% \cmidrule(lr){2-5}
% & \specialcell{on-\\policy\\\cite{mlcad_abc}} & \specialcell{SA+\\Pred.\\\cite{bullseye}} & \specialcell{MCTS\\\cite{neto2022flowtune}} & \specialcell{\textbf{Ours}} \\
% \midrule
% arbiter & \textbf{0.03} & \textbf{0.03} & \textbf{0.03} & \textbf{0.03}\\
% cavlc & 16.28 & 16.75 & 15.85 & \textbf{17.77}\\
% ctrl & 22.97 & 25.85 & 27.58 & \textbf{30.05}\\
% i2c & 14.91 & 13.10 & 13.45 & \textbf{14.95} \\
% int2float & 7.41 & 7.52 & 8.10 & \textbf{10.62}\\
% mem\_ctrl & 22.54 & 21.45 & 21.55 & \textbf{22.75}\\
% priority & 74.62 & 77.10 & \textbf{77.53} & 76.35\\
% router & 10.71 & \textbf{27.53} & 21.63 & 25.53\\
% voter & 8.26 & 26.15 & \textbf{27.10} & \textbf{27.10}\\
% \midrule
% Geomean & 8.29 & 10.47 & 10.38 & \textbf{11.32} \\
% Win ratio & 1/9 & 2/9 & 3/9 & 7/9 \\
% \bottomrule
% \end{tabular}
% }
%     \captionof{table}{Area-delay reduction compared to \texttt{resyn2} on EPFL random-control benchmarks.}% \cmark denotes \solution{} used RL agent during search whereas {\xmark} denotes standard MCTS}
% \label{tab:qorEPFLrc}
% \end{wrapfigure}

==> tables/table_mcnc.tex <==
% \begin{table}[!tbh]
% \centering
% \caption{Area-delay reduction on MCNC benchmarks. \cmark denotes \solution{} used RL agent during search whereas {\xmark} denotes Flowtune (Blind MCTS search). $K$: Number of iterations post which winner thread is picked}
% \label{tab:qorMCNC}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lrrrccccrrrr}
% \toprule
% \multirow{2}{*}{Benchmarks}& \multicolumn{3}{c}{ADP reduction(\%)} & \multicolumn{4}{c}{Pre-trained agent used?} & \multicolumn{4}{c}{ADP reduction(\%)} \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-8} \cmidrule(lr){9-12}
% &  \specialcell{Flowtune} & \specialcell{MCTS\\$+$RL} & \specialcell{Bulls-eye} & \specialcell{Zero\\(cosine)} & \specialcell{Low\\(k=20)} & \specialcell{Mid\\(k=40)} & \specialcell{High\\(k=60)} & \specialcell{Zero\\(cosine)} & \specialcell{Low\\(k=20)} & \specialcell{Mid\\(k=40)} & \specialcell{High\\(k=60)} \\
% \midrule
% alu4 & 17.05 & \textbf{21.95} & 17.58 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{21.95} & \textbf{21.95} &\textbf{21.95}& \textbf{21.95}\\
% apex1 & 15.95 & \textbf{17.54} & 17.01 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{17.54} & \textbf{17.54} & \textbf{17.54} & \textbf{17.54} \\
% apex2 & 13.06 & \textbf{17.51}  & 15.58 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{17.51} & \textbf{17.51} & \textbf{17.51} & \textbf{17.51} \\
% apex4 & 13.01 & \textbf{13.95} & 13.01 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{13.95} & \textbf{13.95} & \textbf{13.95} & \textbf{13.95}\\
% i9 & 46.89 & \textbf{53.97}  & 46.45 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{53.97} & \textbf{53.97} & \textbf{53.97} & \textbf{53.97}\\
% m4 & 14.98 & \textbf{20.05} & 18.16 & {\cmark} & {\xmark} & {\cmark} & {\cmark} & \textbf{20.05} & 14.98 & \textbf{20.05} & \textbf{20.05} \\
% prom1 & 6.50 & \textbf{11.23} & 8.53 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{11.23} & \textbf{11.23} & \textbf{11.23} & \textbf{11.23} \\
% b9 & 23.21 & \textbf{24.10} & 23.65 &{\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{24.10} &\textbf{24.10}& \textbf{24.10}& \textbf{24.10} \\
% c880 & 17.75 & \textbf{24.58} & 19.95 & {\cmark} & {\cmark} & {\cmark} & {\cmark} & \textbf{24.58} & \textbf{24.58} & \textbf{24.58} & \textbf{24.58}  \\
% c7552 & \textbf{20.45} & 12.78 & 17.62 &{\cmark} & {\xmark} & {\xmark} & {\xmark} & 12.78 & \textbf{20.45} & \textbf{20.45} & \textbf{20.45}  \\
% pair & \textbf{13.10} & 12.65 & 10.02 &{\xmark} & {\xmark} & {\xmark} & {\xmark} & \textbf{13.10} & \textbf{13.10} & \textbf{13.10} & \textbf{13.10}  \\
% max1024 & 19.65 & 18.32 & \textbf{20.27} &{\xmark} & {\xmark} & {\xmark} & {\xmark} & 19.65 & 19.65 & 19.65 & 19.65\\
% \midrule
% Geomean & 16.66 & 18.84 & 17.34 & & & & & 19.00 & \textbf{\bt{19.29}} & \textbf{\rt{19.76}} & \textbf{\rt{19.76}} \\
% Win ratio & 2/12 & 9/12 & 1/12 &  &  & & & 10/12 & 10/12 & 11/12 & 11/12\\
% \bottomrule
% \end{tabular}
% }

% \end{table}


% \begin{table}[!tbh]
% \centering
% \caption{Area-delay reduction on MCNC benchmarks. \cmark denotes \solution{} used RL agent during search whereas {\xmark} denotes Flowtune (Blind MCTS search). $K$: Number of iterations post which winner thread is picked}
% \label{tab:qorMCNC}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lrrrrr}
% \toprule
% \multirow{2}{*}{Benchmarks}& \multicolumn{4}{c}{Methods} \\
% \cmidrule(lr){2-6}
% & \specialcell{on-policy} & \specialcell{Bulls-eye} & \specialcell{Flowtune} & \specialcell{MCTS\\$+$RL} & \specialcell{\solution{}} \\
% \midrule
% alu4 & & 17.58 & 17.05 & \textbf{21.95} &  \textbf{21.95}(\cmark) \\
% apex1 & & 17.01 & 15.95 & \textbf{17.54} & \textbf{17.54}(\cmark)\\
% apex2 & & 15.58 & 13.06 & \textbf{17.51} & \textbf{17.51}(\cmark) \\
% apex4 & & 13.01 & 13.01 & \textbf{13.95} & \textbf{13.95}(\cmark) \\
% i9 & & 46.45 & 46.89 & \textbf{53.97} & \textbf{53.97}(\cmark)\\
% m4 & & 18.16 & 14.98 & \textbf{20.05} & \textbf{20.05}(\cmark)\\
% prom1 & & 8.53 & 6.50 & \textbf{11.23} & \textbf{11.23}(\cmark)\\
% b9 & & 23.65 & 23.21 & \textbf{24.10}  &\textbf{24.10}(\cmark)\\
% c880 & & 19.95 & 17.75 & \textbf{24.58} & \textbf{24.58}(\cmark) \\
% c7552 & & 17.62 & \textbf{20.45} & 12.78  & 12.78(\cmark)\\
% pair & & 10.02 & \textbf{13.10} & 12.65 &  \textbf{13.10}(\xmark)\\
% max1024 & & \textbf{20.27} & 19.65 & 18.32 & 19.65(\xmark)\\
% \midrule
% Geomean & & 17.34 & 16.66 & 18.84 & \textbf{19.00} \\
% Win ratio &  & 1/12 & 2/12 & 9/12 & 10/12 \\
% \bottomrule
% \end{tabular}
% }

% \end{table}

\begin{wrapfigure}[20]{r}{0.5\textwidth}
\centering
\setlength\tabcolsep{3.5pt}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lrrrrrr}
\toprule
\multirow{3}{*}{Designs}& \multicolumn{5}{c}{ADP reduction (in \%)} & \multirow{3}{*}{\begin{tabular}{@{}c@{}}Iso-\\ADP\\Speed-\\Up\end{tabular}} \\
\cmidrule(lr){2-6}
& \multirow{2}{*}{\begin{tabular}{@{}c@{}}Online-\\RL\\\cite{mlcad_abc}\end{tabular}}& \multirow{2}{*}{\begin{tabular}{@{}c@{}}SA+\\Pred.\\\cite{bullseye}\end{tabular}} & \multirow{2}{*}{\begin{tabular}{@{}c@{}}MCTS\\\cite{neto2022flowtune}\end{tabular}} &
\multicolumn{2}{c}{\solution{}} & \\
\cmidrule(lr){5-6}
& & & & $\alpha=1$ & +OOD & \\
\midrule
alu4 & 20.61 & 17.58 & 17.05 & \textbf{21.95} &  \textbf{21.95}(\cmark) & 4.5x \\
apex1 & 6.58 & 17.01 & 15.95 & \textbf{17.54} & \textbf{17.54}(\cmark)& 2.6x\\
apex2 & 8.12 & 15.58 & 13.06 & \textbf{17.51} & \textbf{17.51}(\cmark) & 4.7x \\
apex4 & 13.53 & 13.01 & 13.01 & \textbf{13.95} & \textbf{13.95}(\cmark) & 3.2x\\
i9 & 39.35& 46.45 & 46.89 & \textbf{53.97} & \textbf{53.97}(\cmark) & 1.6x\\
m4 & \textbf{20.95} & 18.16 & 14.98 & 20.05 & 20.05(\cmark) & 1.7x \\
prom1 & 4.97& 8.53 & 6.50 & \textbf{11.23} & \textbf{11.23}(\cmark) & 2.5x \\
b9 & 17.92 & 23.65 & 23.21 & \textbf{24.10}  &\textbf{24.10}(\cmark) & 6.3x\\
c880 & 16.23 & 19.95 & 17.75 & \textbf{24.58} & \textbf{24.58}(\cmark) & 6.3x \\
c7552 & 20.21 & 17.62 & \textbf{20.45} & 12.78  & \textbf{20.45}(\xmark) & 1.0x\\
pair & 4.73 & 10.02 & \textbf{13.10} & 12.65 &  \textbf{13.10}(\xmark)& 1.0x\\
max1024 & 11.39 & \textbf{20.27} & 19.65 & 18.32 & 19.65(\xmark) & 1.0x\\
\midrule
Geomean & 12.80 & 17.34 & 16.66 & 18.84 & \textbf{19.76} & 2.5x \\
Win ratio & 1/12 & 1/12 & 2/12 & 8/12 & 10/12 & 9/12\\
\bottomrule
\end{tabular}
}
    \captionof{table}{Area-delay reduction over \texttt{resyn2} on MCNC benchmarks. \cmark denotes \solution{} used RL agent during search whereas {\xmark} denotes standard MCTS}
\label{tab:qorMCNC}
\end{wrapfigure}


% \begin{wrapfigure}{r}{0.4\textwidth}
% \centering
% \setlength\tabcolsep{3.5pt}
% \resizebox{0.4\textwidth}{!}{%
% \begin{tabular}{lrrrr}
% \toprule
% \multirow{2}{*}{Designs}& \multicolumn{3}{c}{ADP reduction (in \%)} \\
% \cmidrule(lr){2-5}
% & \specialcell{on-\\policy\\\cite{mlcad_abc}} & \specialcell{SA+\\Pred.\\\cite{bullseye}} & \specialcell{MCTS\\\cite{neto2022flowtune}} & \specialcell{\textbf{Ours}} \\
% \midrule
% alu4 & 20.61 & 17.58 & 17.05 & \textbf{20.84} \\
% apex1 & 6.58 & 17.01 & 15.95 & \textbf{19.23} \\
% apex2 & 8.12 & 15.58 & 13.06 & \textbf{16.98} \\
% apex4 & 13.53 & 13.01 & 13.01 & \textbf{14.64} \\
% i9 & 39.35& 46.45 & 46.89 & \textbf{52.45} \\
% m4 & \textbf{20.95} & 18.16 & 14.98 & 18.07\\
% prom1 & 4.97& 8.53 & 6.50 & \textbf{12.35}\\
% b9 & 17.92 & 23.65 & 23.21 & \textbf{24.10}\\
% c880 & 16.23 & 19.95 & 17.75 & \textbf{24.70} \\
% c7552 & 20.21 & 17.62 & 20.45 & \textbf{21.12}\\
% pair & 4.73 & 10.02 & 13.10 & \textbf{16.75}\\
% max1024 & 11.39 & 20.27 & 19.65 & \textbf{21.37}\\
% \midrule
% Geomean & 12.80 & 17.34 & 16.66 & \textbf{20.41} \\
% Win ratio & 1/12 & 1/12 & 2/12 & 11/12 \\
% \bottomrule
% \end{tabular}
% }
%     \captionof{table}{Area-delay reduction over \texttt{resyn2} on MCNC benchmarks.}%\cmark denotes \solution{} used RL agent during search whereas {\xmark} denotes standard MCTS}
% \label{tab:qorMCNC}
% \end{wrapfigure}
